A QR Decomposition Approach to Factor Modelling: A Thesis Report

An observed $K$-dimensional series $\left\{ y_{n}\right\} _{n=1}^{N}$ is expressed in terms of a lower $p$-dimensional latent series called factors $f_{n}$ and random noise $\varepsilon_{n}$. The equation, $y_{n}=Qf_{n}+\varepsilon_{n}$ is taken to relate the factors with the observation. The goal is to determine the dimension of the factors, $p$, the factor loading matrix, $Q$, and the factors $f_{n}$. Here, it is assumed that the noise co-variance is positive definite and allowed to be correlated with the factors. An augmented matrix, \[ \tilde{M}\triangleq\left[\begin{array}{cccc} \tilde{\Sigma}_{yy}(1) & \tilde{\Sigma}_{yy}(2) & \ldots & \tilde{\Sigma}_{yy}(m)\end{array}\right] \] is formed using the observed sample autocovariances $\tilde{\Sigma}_{yy}(l)=\frac{1}{N-l}\sum_{n=1}^{N-l}\left(y_{n+l}-\bar{y}\right)\left(y_{n}-\bar{y}\right)^{\top}$, $\bar{y}=\frac{1}{N}\sum_{n=1}^{N}y_{n}$. Estimating $p$ is equated to determining the numerical rank of $\tilde{M}$. Using Rank Revealing QR (RRQR) decomposition, a model order detection scheme is proposed for determining the numerical rank and for estimating the loading matrix $Q$. The rate of convergence of the estimates, as $K$ and $N$ tends to infinity, is derived and compared with that of the existing Eigen Value Decomposition based approach. Two applications of this algorithm, i) The problem of extracting signals from their noisy mixtures and ii) modelling of the S&P index are presented.

==> includes/Chapter-3.tex <==
\selectlanguage{english}%

\chapter{Summary of the Algorithm}

In this chapter, the summary of the algorithm for factor modeling
using QR decomposition is presented.
\begin{enumerate}
\item Let $\left\{ y_{n}\right\} _{n=1}^{N}$ be the observed data. And
the data model is assumed as $y_{n}=Qf_{n}+\varepsilon_{n}$ where
$Q$ is an orthonormal matrix (factor loading matrix) , $f_{n}$ are
factors and $\varepsilon_{n}$ is random noise. 
\item Compute $\tilde{M}\triangleq\left[\begin{array}{cccc}
\tilde{\Sigma}_{yy}(1) & \tilde{\Sigma}_{yy}(2) & \ldots & \tilde{\Sigma}_{yy}(m)\end{array}\right]$ where, $\tilde{\Sigma}_{yy}(l)$ is the sample auto-covariance given
by 
\begin{eqnarray}
\tilde{\Sigma}_{yy}(k) & = & \frac{1}{N-k}\sum_{n=1}^{N-k}\left(y_{n+k}-\bar{y}\right)\left(y_{n}-\bar{y}\right)^{\top},\label{Eqn11a-1}
\end{eqnarray}
where $\bar{y}\triangleq\frac{1}{N}\sum_{t=1}^{N}y_{n}$. 
\item To evaluate the Numerical Rank, $p$, 

\begin{enumerate}
\item Set $i=1$
\item First the permutation matrix $\Pi$ is got by using \noun{Hybrid-III}\emph{
}algorithm\emph{ }assuming a numerical rank of $i$\emph{.}
\item Take Gram-Schmidt QR (GS-QR) decomposition of $\tilde{M}\Pi$ \emph{i.e.,}
$\tilde{M}\Pi=\tilde{Q}\tilde{R}$. Compute 
\[
r_{i}=\frac{\gamma_{i}+\epsilon}{\gamma_{i+1}+\epsilon}
\]
 where $\gamma_{i}$ and $\gamma_{i+1}$ are the $i^{th}$ and $i+1^{th}$
diagonal values of $\tilde{R}$ and $\epsilon=\frac{\gamma_{1}}{\sqrt{KN}}$.
\item Set $i=i+1$
\item \textbf{Repeat Until $i<P$ }where, $P$ is taken such that $p<P$. 
\end{enumerate}
\item Now, estimate of numerical rank, $\hat{p}$, is got by 
\begin{equation}
\hat{p}=\arg\max_{i}\, r_{i},\label{eq:model_order-1}
\end{equation}
. 
\item Evaluate RRQR decomposition of $\tilde{M}$ using \noun{Hybrid-I}
algorithm \cite{chandrasekaran1994rank} presented in \emph{Algorithm
2. }Let the RRQR Decomposition be as in 
\begin{eqnarray}
\tilde{M}\Pi & = & \left[\begin{array}{cc}
\tilde{M}_{p} & \tilde{M}_{mK-p}\end{array}\right]\nonumber \\
 & = & \left[\begin{array}{cc}
\mathcal{\tilde{Q}}_{p} & \tilde{\mathcal{Q}}_{K-p}\end{array}\right]\left[\begin{array}{cc}
\tilde{R}_{11} & \tilde{R}_{12}\\
0 & \tilde{R}_{22}
\end{array}\right]\nonumber \\
 & = & \mbox{\ensuremath{\mathcal{\tilde{Q}}}}\tilde{R},\label{eq:rrqr1-1-1}
\end{eqnarray}
 
\item Now, the finite sample estimate of $\hat{Q}$ is got by, $\hat{Q}_{N,K}=\tilde{Q}(:,1:\hat{p})$.
\item Finally the estimate of factors is got by, $\hat{f}_{n}=\hat{Q}_{N,K}^{\top}y_{n}$.
\end{enumerate}
The \emph{QR-CP }algorithm can be found in \cite{golub2012matrix,chandrasekaran1994rank},
while the \noun{Hybrid-I}\emph{ }RRQR algorithm is presented in \cite{chandrasekaran1994rank}.
Here, for the sake of completion, \emph{QR-CP }algorithm and the \noun{Hybrid
I,II}\emph{ }and\emph{ }\noun{III}\emph{ RRQR }algorithms are presented
in detail in \emph{Algorithm 1,2,3 \& 4 }respectively. 

\begin{algorithm}
\caption{QR Decomposition with Column Pivoting}
~\\
~
\begin{enumerate}
\item The matrix to be decomposed be $\tilde{M}\in\mathbb{R}^{K,mK}$.
\item Let the permutation matrix $\Pi$ be initialized as an Identity matrix
of order $mK$.
\item Take a value of $P$ such that, $p<P<\min(K,N)$
\item Take Gram-Schmidt QR (GS-QR) decomposition of $\tilde{M}$ i.e., $\tilde{M}=Q^{(0)}R^{(0)}$,
where $R^{(s)}\triangleq\begin{array}{cc}
 & \begin{array}{cc}
s\quad\; & mK-s\end{array}\\
\begin{array}{c}
s\\
K-s
\end{array} & \left[\begin{array}{cc}
R_{11}^{(s)}\qquad & R_{12}^{(s)}\\
0\qquad & R_{22}^{(s)}
\end{array}\right]
\end{array}$ and set $s=0.$ 
\item \textbf{Repeat} \\
~

\begin{enumerate}
\item Let $e_{i}$ be the $i^{th}$ column of an identity matrix of order
$mK-s$.
\item $j\triangleq\arg\max_{1\leq i\leq mK-s}\left\Vert R_{22}^{(s)}e_{i}\right\Vert _{2}$
\item Interchange the columns $j$ and $s+1$ in $\Pi$.
\item Compute, GS-QR of $\tilde{M}\Pi$ as $\tilde{M}\Pi\triangleq Q^{(s)}R^{(s)}$
\item $s=s+1$
\end{enumerate}
\item \textbf{Until} $s>P$
\item Return $\Pi$\end{enumerate}
\end{algorithm}


\begin{algorithm}
\caption{\noun{Hybrid-I} algorithm of RRQR}
~\\
~
\begin{enumerate}
\item The Matrix to be decomposed is got as $\tilde{M}\in\mathbb{R}^{K\times Km}$.
The numerical rank, $\hat{p}$, is got by using \emph{Algorithm 1
}and (\ref{eq:model_order}). 
\item Using the $\Pi$ \emph{Algorithm 1}, apply QR-GS to $\tilde{M}\Pi$
as $\tilde{M}\Pi=\bar{Q}\bar{R}$ and set $s=0$; 

\begin{enumerate}
\item \textbf{Repeat}\\
\textbf{~}

\begin{enumerate}
\item Set $permuted=0$. 
\item Let $\bar{R}^{(s)}\triangleq\begin{array}{cc}
 & \begin{array}{cc}
\hat{p}-1\quad\; & mK-\hat{p}+1\end{array}\\
\begin{array}{c}
\hat{p}-1\\
K-\hat{p}+1
\end{array} & \left[\begin{array}{cc}
\bar{R}_{11}^{(s)}\qquad & \bar{R}_{12}^{(s)}\\
0\qquad & \bar{R}_{22}^{(s)}
\end{array}\right]
\end{array}$
\item Let $e_{i}$ be the $i^{th}$ column of an identity matrix of order
$mK-\hat{p}+1$.
\item Let\textbf{ }$j\triangleq\arg\max_{1\leq i\leq mK-\hat{p}+1}\left\Vert \bar{R}_{22}^{(s)}e_{i}\right\Vert _{2}$
\item \textbf{If $j\neq1$ then}\\
\textbf{~}

\begin{enumerate}
\item $permuted$= 1
\item Interchange columns $\hat{p}+j-1$ and $\hat{p}$ in $\Pi$.
\item apply QR-GS to $\tilde{M}\Pi$ to get new $\bar{Q}\bar{R}$.
\end{enumerate}
\item Now divide $\bar{R}$ as $\bar{R}^{(s)}\triangleq\begin{array}{cc}
 & \begin{array}{cc}
\hat{p}\quad\; & mK-\hat{p}\end{array}\\
\begin{array}{c}
\hat{p}\\
K-\hat{p}
\end{array} & \left[\begin{array}{cc}
\bar{R}_{11}^{(s)}\qquad & \bar{R}_{12}^{(s)}\\
0\qquad & \bar{R}_{22}^{(s)}
\end{array}\right]
\end{array}$and Let $e_{i}$ be the $i^{th}$ column of an identity matrix of
order $\hat{p}$.
\item Let $j\triangleq\arg\max_{1\leq i\leq\hat{p}}\left\Vert e_{i}^{\top}\bar{R}_{11}^{(s)-1}\right\Vert $
\item \textbf{If $j\neq\hat{p}$ then}\\
\textbf{~}

\begin{enumerate}
\item $permuted=1$
\item Exchange columns $j$ and $\hat{p}$ in $\Pi$
\item apply QR-GS to $\tilde{M}\Pi$ to get new $\bar{Q}^{(s)}\bar{R}^{(s)}$.
\item $s=s+1$
\end{enumerate}
\end{enumerate}
\item \textbf{Until $permuted\neq0$}
\item Now RRQR decomposition is given by taking GS-QR of $\tilde{M}\Pi$
as, $\tilde{M}\Pi=\tilde{Q}\tilde{R}$\end{enumerate}
\end{enumerate}
\end{algorithm}


\begin{algorithm}
\caption{\noun{Hybrid-I}I algorithm of RRQR}
~\\
~
\begin{enumerate}
\item The Matrix to be decomposed is got as $\tilde{M}\in\mathbb{R}^{K\times Km}$.
The numerical rank is assumed as, $\hat{p}$. 
\item Using the $\Pi$ from \emph{Algorithm 1}, apply QR-GS to $\tilde{M}\Pi$
as $\tilde{M}\Pi=\bar{Q}\bar{R}$ and set $s=0$; 

\begin{enumerate}
\item \textbf{Repeat}\\
\textbf{~}

\begin{enumerate}
\item Set $permuted=0$. 
\item Let $\bar{R}^{(s)}\triangleq\begin{array}{cc}
 & \begin{array}{cc}
\hat{p}\quad\; & mK-\hat{p}\end{array}\\
\begin{array}{c}
\hat{p}\\
K-\hat{p}
\end{array} & \left[\begin{array}{cc}
\bar{R}_{11}^{(s)}\qquad & \bar{R}_{12}^{(s)}\\
0\qquad & \bar{R}_{22}^{(s)}
\end{array}\right]
\end{array}$
\item Let $e_{i}$ be the $i^{th}$ column of an identity matrix of order
$mK-\hat{p}$.
\item Let\textbf{ }$j\triangleq\arg\max_{1\leq i\leq mK-\hat{p}}\left\Vert \bar{R}_{22}^{(s)}e_{i}\right\Vert _{2}$
\item \textbf{If $j\neq1$ then}\\
\textbf{~}

\begin{enumerate}
\item $permuted$= 1
\item Interchange columns $\hat{p}+j$ and $\hat{p}+1$ in $\Pi$.
\item apply QR-GS to $\tilde{M}\Pi$ to get new $\bar{Q}\bar{R}$.
\end{enumerate}
\item Now divide $\bar{R}$ as $\bar{R}^{(s)}\triangleq\begin{array}{cc}
 & \begin{array}{cc}
\hat{p}+1\quad\; & mK-\hat{p}-1\end{array}\\
\begin{array}{c}
\hat{p}+1\\
K-\hat{p}-1
\end{array} & \left[\begin{array}{cc}
\bar{R}_{11}^{(s)}\qquad & \bar{R}_{12}^{(s)}\\
0\qquad & \bar{R}_{22}^{(s)}
\end{array}\right]
\end{array}$and Let $e_{i}$ be the $i^{th}$ column of an identity matrix of
order $\hat{p}$.
\item Let $j\triangleq\arg\max_{1\leq i\leq\hat{p}+1}\left\Vert e_{i}^{\top}\bar{R}_{11}^{(s)-1}\right\Vert $
\item \textbf{If $j\neq\hat{p}+1$ then}\\
\textbf{~}

\begin{enumerate}
\item $permuted=1$
\item Exchange columns $j$ and $\hat{p}+1$ in $\Pi$
\item apply QR-GS to $\tilde{M}\Pi$ to get new $\bar{Q}^{(s)}\bar{R}^{(s)}$.
\item $s=s+1$
\end{enumerate}
\end{enumerate}
\item \textbf{Until $permuted\neq0$}
\item Now RRQR decomposition is given by taking GS-QR of $\tilde{M}\Pi$
as, $\tilde{M}\Pi=\tilde{Q}\tilde{R}$\end{enumerate}
\end{enumerate}
\end{algorithm}


\begin{algorithm}
\caption{\noun{Hybrid-I}II Algorithm}
~\\
~
\begin{enumerate}
\item \textbf{Repeat}

\begin{enumerate}
\item \noun{Hybrid-I}
\item \noun{Hybrid-I}I
\end{enumerate}
\item \textbf{Until }no permutations occur\end{enumerate}
\end{algorithm}
\selectlanguage{british}%


